Study of Compact Stars and their Properties based on General Relativistic Core-Envelope Models

This thesis explores compact objects, particularly neutron stars, focusing on their properties, classification, and stability within the framework of general relativity. Two distinct studies are presented. The first study examines the properties of compact stars, including neutron stars, using an equation of state from a core-envelope model. By solving Einstein's equations with pseudo-spheroidal and spherically symmetric geometries, the mass-radius relationship is derived, leading to the classification of compact stars into three categories: highly compact self-bound stars (radii $<$ 9 km), normal neutron stars (radii 9--12 km), and soft matter neutron stars (radii 12--20 km). Other parameters such as Keplerian frequency, surface gravity, and gravitational redshift are also computed, offering insights into highly compact neutron stars with exotic compositions. The second study investigates the impact of density perturbations and local anisotropy on stellar stability. Using the cracking concept and a core-envelope model with anisotropic pressure in the envelope, we explore the potential of these configurations as progenitors for starquakes. The buildup of strain energy in the envelope, linked to anisotropy, can reach up to $10^{50}$ erg -- comparable to energy released in giant gamma-ray bursts. This study thus contributes to understanding the relationship between starquakes and gamma-ray bursts. Overall, this work advances the understanding of neutron stars by classifying them based on their radii and investigating the stability of their matter structures, providing new insights into starquakes and their possible connections with gamma-ray bursts.

==> frontmatter/Acknowledgments.tex <==
%*******************************************************
% Publications
%*******************************************************
\pdfbookmark[1]{Acknowledgements}{Acknowledgements}

% \begin{flushright}{\slshape    
%     We have seen that \sout{computer programming} physics is an art, \\ 
%     because it applies accumulated knowledge to the world, \\ 
%     because it requires skill and ingenuity, and especially \\
%     because it produces objects of beauty.} \\ \medskip
%     --- Adapted from \defcitealias{knuth:1974}{Donald E. Knuth}\citetalias{knuth:1974} \citep{knuth:1974}
% \end{flushright}

\bigskip

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax


\chapter*{Acknowledgements}

``\textit{It has become almost a cliche to remark that nobody boasts of ignorance of literature, but it is socially acceptable to boast ignorance of science and proudly claim incompetence in mathematics.}''                                
\begin{flushright}
-- Richard Dawkins
\end{flushright}


\bigskip

 First and foremost, I want to thank my supervisor, Prof. P. C. Vinodkumar, who has been an excellent mentor during my years as a PhD student. He is an extremely wise, enthusiastic, supportive, and tolerant person, and I owe him immeasurable thanks for making me realize the value of critical and independent thinking. To say that he has taught me how theoretical physics is done, would be an understatement. Vinodkumar, it has been a pleasure working with you, and I am truly honored to be your last PhD student.
 
 
    I am grateful to Prof. V. O. Thomas and Dr. Bharat Ratanpal for hours of invigorating discussions on several aspects of Compact objects and mathematical relativity ranging from stability, differential geometry  and geometry of spacetime. I am also thankful to Thomas for sharing his  insights in analytical calculations that resulted in a number of fruitful collaborations during my PhD.


    I am profoundly grateful for the invaluable support and guidance of Yavuz Eksi throughout my research journey. Our discussions on spacetime geometry and the gravity of compact stars have significantly shaped my understanding of these complex topics. His expertise and willingness to share his knowledge in tensor and differential geometry have been instrumental in advancing my research.

  I would like to express my deepest gratitude to Prof. J. N. Pandya for providing me with the necessary infrastructure and support throughout the time I spent working on my thesis.

    I would like to extend my heartfelt gratitude to Prof. Pankaj Joshi, the Director of the International Center for Cosmology (ICC) at Charusat, for his invaluable support, exceptional facilities, and warm hospitality during my visit. I would also like to express my appreciation to my colleagues and friends at Charusat, Parth, Dipanjan, Ashwathi, Vishwa, and Tapobroto. Their friendship and encouragement have provided a sense of belonging and motivation throughout my time at the ICC.

I would like to express my sincere appreciation to two dear friends, Swagat Mishra and Ekta Shah, whose friendship and intellectual discussions have enriched my scientific journey, particularly in the field of cosmology and science as a whole.

    I would like to extend my heartfelt appreciation to my dear friends Kamal, Jayraj, Gaurav, who have been an integral part of my academic journey in the Department of Physics. Our thought-provoking discussions and debates on various topics, including politics, history, physics, mathematics, and philosophy, have profoundly enriched my research and personal growth. 

    I would like to express my sincere gratitude to Sagar Soni and Ahmed Al-Haysah from the Department of Mathematics. I am immensely grateful for the invaluable discussions we have had on topics related to mathematical relativity and differential geometry. Their deep knowledge and insightful perspectives have greatly enriched my understanding of these complex subjects. 
 
I would like to express my heartfelt gratitude to my dear friends Bhavesh Socha,  Hitesh Bhoi, Keyur Sangani, Piyush Rajput, Alkesh Patel, Payal Chauhan, Hiren Jagani, Kaushik Jodhani, Atish Dhameliya, Tejas Jani, Sharon Christian, Mohammed Dawood, Kajal Thakar, Bhavik Moradiya, Rahul MJ, Parth Pattani, Chaitanya Raval, Ridhhi Patel, Yesha Sharma, Priyanka Parmar, Nishita Pathak, Bhoomika Pandya, and others who have enlightened my life in Vallabh Vidyanagar and made it less lonely. Your friendship and presence have been a tremendous source of joy, support, and inspiration throughout my time in Vallabh Vidyanagar. The countless moments we shared, the laughter we enjoyed, and the memories we created have made this journey unforgettable.


Dhaval and Mitali, your friendship and kindness have meant the world to me. Beyond the academic realm, I am grateful for the love and care you have extended to me as a member of your family. Your willingness to share your lives, traditions, and celebrations has made me feel embraced and cherished. The moments we have shared together have created lasting memories that I will treasure forever.

I would like to express my deepest gratitude to my loving family for their unwavering support and sacrifices throughout my educational journey. My heartfelt appreciation goes to my father, Chatur, and my mother, Mamta, whose dedication and selflessness have been instrumental in shaping my academic pursuits. Their unconditional love, encouragement, and belief in my abilities have been a constant source of inspiration.
I am immensely grateful for the pivotal role played by my brother, Nevil, and my sisters, Chetna, Payal and Mayuri  who have been a constant source of love, inspiration, and support. Their encouragement, understanding, and shared experiences have been invaluable throughout my academic journey. I am thankful  to my brothers-in-law, Rakesh Bavishi, Jasmin Limbasiya, and Khushal Malani, for their invaluable financial support throughout my Ph.D. journey. Their generosity and belief in my academic pursuits have played a significant role in enabling me to achieve my goals.

I would like to make a special mention of my partner, Megha, whose unwavering support and understanding have been a constant source of strength and motivation throughout this demanding journey. Her patience, encouragement, and love have sustained me during the challenging times, and I am deeply thankful for her presence in my life.


I am deeply grateful to the great many people who have played significant roles in my journey from a small town Gujarati medium primary school to the completion of my Ph.D. in Physics. I would like to extend my sincere appreciation to all those who have supported and contributed to my career. I apologize in advance if I have unintentionally overlooked anyone in this acknowledgment, as each person's contribution has been invaluable.




\endgroup

==> frontmatter/Certificate_signed.tex <==
\begin{figure*}
    \hspace*{-1.0cm}
    \centering
    \includegraphics[scale=1.1]{frontmatter/Certificate.pdf}
    %\caption{}
\end{figure*}

==> frontmatter/Declaration_signed.tex <==
\begin{figure*}
    %\hspace*{-1.2cm}
    \centering
    \includegraphics[scale=1.0]{frontmatter/Declaration.pdf}
    %\caption{}
\end{figure*}

==> frontmatter/fron.tex <==
\begin{figure*}
    \hspace*{-1.0cm}
    \centering
    \includegraphics[width=18cm,height=34cm]{frontmatter/astronomy (5).png}
    %\caption{}
\end{figure*}
